Modified symmetry technique for mitigation of flow leak near corners for compressible inviscid fluid flow

Using the standard symmetry technique for applying boundary conditions for free slip and flat walls with corners will lead to flow leak through the wall near corners (violation of no penetration condition) and a corresponding error in prediction of pressure. Also, prescribing a state at the corner as a boundary condition is not possible. In this paper, a method for tackling the `corner point state' problem is given and modifications to the standard symmetry technique are proposed to mitigate flow leak near the corner. Using this modified symmetry technique, numerical solutions to the Euler equations for flows over forward facing and backward facing step are computed employing the Shu-Osher conservative finite difference scheme with WENO-NP3 reconstruction (with a formal order of accuracy in space of 3), Lax-Freidrichs flux splitting, and TVD-RK3 time discretisation. It is shown that using this modified symmetry technique leads to mitigation of flow leak near the corner and a better prediction of shock structure even on coarse meshes.

==> elsarticle/doc/tmp.tex <==
 \begin{enumerate}[Step 1.]
  \item This is the first step of the example list.
  \item Obviously this is the second step.
  \item The final step to wind up this example.
 \end{enumerate}

